Template bank for sub solar mass compact binary mergers in the fourth observing run of Advanced LIGO, Advanced Virgo, and KAGRA

Matched-filtering searches for gravitational-wave signals from compact binary mergers employ template banks which are a collection of modeled waveforms described by unique intrinsic parameters. We present two banks designed for low-latency and archive sub-solar mass (SSM) searches in data from the fourth observing run of LIGO-Virgo-KAGRA, and demonstrate the efficacy of the banks via simulated signals. Further, we introduce a set of modifications to the geometric, manifold algorithm that allow the method to work for exceedingly low component masses necessary for SSM bank production. The archive search bank contains a total of $3,452,006$ templates, and covers a mass parameter space of $0.2$ to $10\ M_\odot$ in the larger component and $0.2$ to $1.0\ M_\odot$ in the smaller component, the spin parameter space of $-0.9$ to $0.9$ for masses above $0.5$ $M_\odot$ and $-0.1$ to $0.1$ for masses below $0.5$ $M_\odot$, and the mass ratio parameter space of $1$ to $10$. The PSD used was from a week of the first half of the fourth observing run of Advanced LIGO, Advanced Virgo, and KAGRA, and the low frequency cutoff was set to $45$ Hz with a maximum waveform duration of $128$ seconds. The bank simulations performed using SBank have shown that the banks presented in this paper have sufficient efficacy for use in their respective searches.

==> Makefile <==
filename = paper
TEXFILES = *tex

all: pdf

pdf:
	latexmk -pdf ${filename}

clean:
	rm -f *.pdf *.aux *.bbl *.blg *.log *.toc *.out *Notes.bib *.fdb* *.fls gitID.txt

arxiv.tar: ${filename}.pdf $(TEXFILES)
	tar chvf arxiv.tar $(TEXFILES) ${filename}.bbl $$(grep includegraphic $(TEXFILES) | egrep -o '\{.*\}' | sed 's/{//' | sed 's/}//')


==> scripts/offline_ssm_bank/sbank_plot_sim_ssm_offline <==
# Copyright (C) 2011  Nickolas Fotopoulos
# Copyright (C) 2011-2017  Stephen Privitera
#
# This program is free software; you can redistribute it and/or modify it
# under the terms of the GNU General Public License as published by the
# Free Software Foundation; either version 2 of the License, or (at your
# option) any later version.
#
# This program is distributed in the hope that it will be useful, but
# WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the GNU General
# Public License for more details.
#
# You should have received a copy of the GNU General Public License along
# with this program; if not, write to the Free Software Foundation, Inc.,
# 51 Franklin Street, Fifth Floor, Boston, MA  02110-1301, USA.

from __future__ import division
from math import ceil, floor, log10
import sys
import os
import warnings
import numpy as np
import matplotlib
matplotlib.use("Agg")
import matplotlib.pyplot as plt
#plt.rcParams["font.family"] = "serif"
plt.rcParams.update({"font.family": 'serif', 'font.size':10})
plt.rcParams['figure.figsize'] = [4, 3]
plt.rcParams['figure.dpi'] =  300
plt.rcParams['savefig.dpi'] = 300
from lalsimulation import SimInspiralTaylorF2ReducedSpinComputeChi, SimIMRPhenomBComputeChi, SimIMRSEOBNRv4ROMTimeOfFrequency

from h5py import File as H5File

warnings.warn(
    "this script has been moved into the independent `sbank` project, "
    "see https://pypi.org/project/sbank/ for details, and will be "
    "removed from lalapps in an upcoming release",
    DeprecationWarning,
)


def find_process_id(process_table, prog_name):
    for program, pid in process_table["program", "process_id"]:
        if program == prog_name:
            return pid
    return None

def find_process_param(pp_table, process_id, param):
    for pid, row_param, value in pp_table["process_id", "param", "value"]:
        if pid == process_id and row_param == param:
            return value

# grab data
match = None

for fname in sys.argv[1:]:
    with H5File(fname, "r") as h5file:

        if match is None:
            match = np.array(h5file["/match_map"])
            inj_arr = np.array(h5file["/sim_inspiral"])
            tmplt_arr = np.array(h5file["/sngl_inspiral"])

        else:
            match = np.concatenate((np.array(h5file["/match_map"]), match))
            tmplt_arr = np.concatenate((np.array(h5file["/sngl_inspiral"]), tmplt_arr))
            inj_arr = np.concatenate((np.array(h5file["/sim_inspiral"]), inj_arr))

inj_sigmasq = match["inj_sigmasq"]
match = match["match"]

order = match.argsort()[::-1]
match = match[order]
inj_arr = inj_arr[order]
tmplt_arr = tmplt_arr[order]

inj_approx = "FIXME"
tmplt_approx = "FIXME"
flow = 45 # FIXME

# derived quantities
# NB: Named fields in dtypes (see ligolw_table_to_array in lalapps_cbc_sbank_sim)
# allow dict-like access to columns: e.g. arr["mass1"].
min_match = match[int(floor(len(match)*0.9))]
inj_M = inj_arr["mass1"] + inj_arr["mass2"] #total mass
inj_Mc = ((inj_arr["mass1"] * inj_arr["mass2"])**0.6) / ((inj_arr["mass1"] + inj_arr["mass2"])**0.2)
inj_eta = inj_arr["mass1"] * inj_arr["mass2"] / (inj_arr["mass1"] + inj_arr["mass2"])**2
tmplt_M = tmplt_arr["mass1"] + tmplt_arr["mass2"]
tmplt_eta = tmplt_arr["mass1"] * tmplt_arr["mass2"] / (tmplt_arr["mass1"] + tmplt_arr["mass2"])**2
inj_mass_ratio = inj_arr["mass1"] / inj_arr["mass2"]

#
# compute effective/reduced spin parameter for templates
#
if tmplt_approx == "TaylorF2RedSpin":
    tmplt_chi_label = "\chi_\mathrm{red}"
    tmplt_chi = [SimInspiralTaylorF2ReducedSpinComputeChi(float(row["mass1"]), float(row["mass2"]), float(row["spin1z"]), float(row["spin2z"])) for row in tmplt_arr]
else: # default to effective spin
    tmplt_chi_label = "\chi_\mathrm{eff}"
    tmplt_chi = [SimIMRPhenomBComputeChi(float(row["mass1"]), float(row["mass2"]), float(row["spin1z"]), float(row["spin2z"])) for row in tmplt_arr]

# FIXME hack
# inj_dur = [SimIMRSEOBNRv4ROMTimeOfFrequency(flow, float(row["mass1"]) * MSUN_SI, float(row["mass2"]) * MSUN_SI, float(row["spin1z"]), float(row["spin2z"])) for row in inj_arr]


#
# compute effective/reduced spin parameter for injections
#
if inj_approx == "TaylorF2RedSpin" or "SpinTaylorT5" in inj_approx: # reduced spin
    inj_chi_label = "\chi_\mathrm{red}"
    inj_chi = [SimInspiralTaylorF2ReducedSpinComputeChi(float(row["mass1"]), float(row["mass2"]), float(row["spin1z"]), float(row["spin2z"])) for row in inj_arr]
elif "SpinTaylorT4" in inj_approx: # reduced spin (requires coordinate transformation)
    inj_chi_label = "\chi_\mathrm{red}"
    chi1 = [row["spin1x"] *np.sin(row["inclination"]) + row["spin1z"] *np.cos(row["inclination"]) for row in inj_arr]
    chi2 = [row["spin2x"] *np.sin(row["inclination"]) + row["spin2z"] *np.cos(row["inclination"]) for row in inj_arr]
    inj_chi = [SimIMRPhenomBComputeChi(float(row["mass1"]), float(row["mass2"]), s1z, s2z) for row, s1z, s2z in zip(inj_arr, chi1, chi2)]
else: # default to effective spin
    inj_chi_label = "\chi_\mathrm{eff}"
    inj_chi = [SimIMRPhenomBComputeChi(float(row["mass1"]), float(row["mass2"]), float(row["spin1z"]), float(row["spin2z"])) for row in inj_arr]

    # IMRPhenomP uses yet another coordinate convention
    if inj_approx == "IMRPhenomP":
        inj_chi *= np.cos(inj_arr["inclination"])


smallest_match = match.min()

from matplotlib.figure import Figure
from matplotlib.backends.backend_agg import FigureCanvasAgg as FigureCanvas

# FIXME
NAME = 'SSM_OFFLINE_LOW_LOW'
# BNS_LOW/BNS_HIGH (SSM_OFFLINE_BNS_LOW): 
# MAX_MISMATCH = 0.6
# NSBH_LOW/NSBH_HIGH: 
# MAX_MISMATCH = 1.0
# HIGH_HIGH:
# MAX_MISMATCH = 0.25
# HIGH_LOW:
# MAX_MISMATCH = 0.25
# LOW_LOW:
MAX_MISMATCH = 0.25

import numpy
mismatch = 1 - match
mismatch_mapped = mismatch
mismatch_mapped[mismatch_mapped < 0.01] = 0.01

# plots

fig = Figure()
ax = fig.add_subplot(111)
collection = ax.scatter(inj_Mc, inj_chi, c=mismatch_mapped, cmap="cividis_r", s=4., linewidth=0, alpha=0.5, norm=matplotlib.colors.LogNorm(0.0+numpy.power(10,-2.0), MAX_MISMATCH))
ax.set_xlabel("Injected Chirp Mass", fontsize=12)
ax.set_ylabel("Injected $%s$" % inj_chi_label, fontsize=12)
ax.tick_params(axis='x', labelsize=12)
ax.tick_params(axis='y', labelsize=12)
ax.grid(True)
# BNS_HIGH:
# ax.set_xlim([0.75, 2.75])
# ax.set_ylim([-0.51, 0.51])
# BNS_LOW:
# ax.set_xlim([0.75, 2.75])
# ax.set_ylim([-0.055, 0.055])
# NSBH_LOW/NSBH_HIGH:
# ax.set_xlim([1.35, 4.75])
# ax.set_ylim([-1.05, 1.05])
# HIGH_HIGH:
# ax.set_xlim([0.4, 2.5])
# ax.set_ylim([-0.95, 0.95])
# HIGH_LOW:
# ax.set_xlim([0.25, 1.25])
# ax.set_ylim([-0.85, 0.85])
# LOW_LOW:
ax.set_xlim([0.165, 0.44])
ax.set_ylim([-0.105, 0.105])
ax.margins(x=1.0,y=1.0)
cbar = fig.colorbar(collection, ax=ax)
cbar.mappable.set_clim(vmin=0.01, vmax=MAX_MISMATCH)
cbar.set_label("mismatch (= 1 - fitting factor)")
canvas = FigureCanvas(fig)
fig.savefig(NAME+"_match_vs_injMc_vs_injchi.png", bbox_inches='tight') 

fig = Figure()
ax = fig.add_subplot(111)
collection = ax.scatter(inj_arr["mass1"], inj_arr["mass2"], c=mismatch_mapped, cmap="cividis_r", s=4., linewidth=0, alpha=0.5, norm=matplotlib.colors.LogNorm(0.0+numpy.power(10,-2.0), MAX_MISMATCH))
ax.set_xlabel("Injected $m_1$ ($M_\odot$)", fontsize=12)
ax.set_ylabel("Injected $m_2$ ($M_\odot$)", fontsize=12)
ax.tick_params(axis='x', labelsize=12)
ax.tick_params(axis='y', labelsize=12)
ax.grid(True)
# BNS_HIGH:
# ax.set_xlim([0.95, 3.05])
# ax.set_ylim([0.95, 3.05])
# BNS_LOW:
# ax.set_xlim([0.95, 3.05])
# ax.set_ylim([0.95, 3.05])
# NSBH_HIGH:
# ax.set_xlim([2.95, 10.05])
# ax.set_ylim([0.95, 3.05])
# NSBH_LOW:
# ax.set_xlim([2.95, 10.05])
# ax.set_ylim([0.95, 3.05])
# HIGH_HIGH:
# ax.set_xlim([0.3, 10.2])
# ax.set_ylim([0.48, 1.02])
# HIGH_LOW:
# ax.set_xlim([0.4, 5.1])
# ax.set_ylim([0.19, 0.51])
# LOW_LOW:
ax.set_xlim([0.19, 0.51])
ax.set_ylim([0.19, 0.51])
ax.margins(x=1.0,y=1.0)
cbar = fig.colorbar(collection, ax=ax)
cbar.mappable.set_clim(vmin=0.01, vmax=MAX_MISMATCH)
cbar.set_label("mismatch (= 1 - fitting factor)")
canvas = FigureCanvas(fig)
fig.savefig(NAME+"_match_vs_injm1_vs_injm2.png", bbox_inches='tight') 

fig = Figure()
ax = fig.add_subplot(111)
collection = ax.scatter(inj_mass_ratio, inj_chi, c=mismatch_mapped, cmap="cividis_r", s=4., linewidth=0, alpha=0.5, norm=matplotlib.colors.LogNorm(0.0+numpy.power(10,-2.0), MAX_MISMATCH))
ax.set_xlabel("Injected mass ratio $q$", fontsize=12)
ax.set_ylabel("Injected $%s$" % inj_chi_label, fontsize=12)
ax.tick_params(axis='x', labelsize=12)
ax.tick_params(axis='y', labelsize=12)
ax.grid(True)
# BNS_HIGH:
# ax.set_xlim([0.95, 3.05])
# ax.set_ylim([-0.51, 0.51])
# BNS_LOW:
# ax.set_xlim([0.95, 3.05])
# ax.set_ylim([-0.055, 0.055])
# NSBH_HIGH:
# ax.set_xlim([0.95, 10.05])
# ax.set_ylim([-1.05, 1.05])
# NSBH_LOW:
# ax.set_xlim([0.95, 10.05])
# ax.set_ylim([-1.05, 1.05])
# HIGH_HIGH:
# ax.set_xlim([0.95, 10.05])
# ax.set_ylim([-0.95, 0.95])
# HIGH_LOW:
# ax.set_xlim([0.95, 10.05])
# ax.set_ylim([-0.95, 0.95])
# LOW_LOW:
ax.set_xlim([0.98, 2.52])
ax.set_ylim([-0.105, 0.105])
ax.margins(x=1.0,y=1.0)
cbar = fig.colorbar(collection, ax=ax)
cbar.mappable.set_clim(vmin=0.01, vmax=MAX_MISMATCH)
cbar.set_label("mismatch (= 1 - fitting factor)")
canvas = FigureCanvas(fig)
fig.savefig(NAME+"_match_vs_injq_vs_injchi.png", bbox_inches='tight') 



==> scripts/offline_ssm_bank/sbank_plot_sim_ssm_offline_cumulative <==
# Copyright (C) 2011  Nickolas Fotopoulos
# Copyright (C) 2011-2017  Stephen Privitera
#
# This program is free software; you can redistribute it and/or modify it
# under the terms of the GNU General Public License as published by the
# Free Software Foundation; either version 2 of the License, or (at your
# option) any later version.
#
# This program is distributed in the hope that it will be useful, but
# WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the GNU General
# Public License for more details.
#
# You should have received a copy of the GNU General Public License along
# with this program; if not, write to the Free Software Foundation, Inc.,
# 51 Franklin Street, Fifth Floor, Boston, MA  02110-1301, USA.

from __future__ import division
from math import ceil, floor, log10
import sys
import os
import warnings
import numpy as np
import matplotlib
matplotlib.use("Agg")
import matplotlib.pyplot as plt
#plt.rcParams["font.family"] = "serif"
plt.rcParams.update({"font.family": 'serif', 'font.size':10})
plt.rcParams['figure.figsize'] = [4, 3]
plt.rcParams['figure.dpi'] =  300
plt.rcParams['savefig.dpi'] = 300
from lalsimulation import SimInspiralTaylorF2ReducedSpinComputeChi, SimIMRPhenomBComputeChi, SimIMRSEOBNRv4ROMTimeOfFrequency

from h5py import File as H5File

warnings.warn(
    "this script has been moved into the independent `sbank` project, "
    "see https://pypi.org/project/sbank/ for details, and will be "
    "removed from lalapps in an upcoming release",
    DeprecationWarning,
)


def find_process_id(process_table, prog_name):
    for program, pid in process_table["program", "process_id"]:
        if program == prog_name:
            return pid
    return None

def find_process_param(pp_table, process_id, param):
    for pid, row_param, value in pp_table["process_id", "param", "value"]:
        if pid == process_id and row_param == param:
            return value

# grab data
match = None
for fname in sys.argv[1:]:
    with H5File(fname, "r") as h5file:

        if match is None:
            match = np.array(h5file["/match_map"])
            inj_arr = np.array(h5file["/sim_inspiral"])
            tmplt_arr = np.array(h5file["/sngl_inspiral"])

        else:
            match = np.concatenate((np.array(h5file["/match_map"]), match))
            tmplt_arr = np.concatenate((np.array(h5file["/sngl_inspiral"]), tmplt_arr))
            inj_arr = np.concatenate((np.array(h5file["/sim_inspiral"]), inj_arr))

inj_sigmasq = match["inj_sigmasq"]
match = match["match"]

order = match.argsort()[::-1]
match = match[order]
inj_arr = inj_arr[order]
tmplt_arr = tmplt_arr[order]

inj_approx = "FIXME"
tmplt_approx = "FIXME"
flow = 45 # FIXME

# derived quantities
# NB: Named fields in dtypes (see ligolw_table_to_array in lalapps_cbc_sbank_sim)
# allow dict-like access to columns: e.g. arr["mass1"].
min_match = match[int(floor(len(match)*0.9))]
inj_M = inj_arr["mass1"] + inj_arr["mass2"] #total mass
inj_Mc = ((inj_arr["mass1"] * inj_arr["mass2"])**0.6) / ((inj_arr["mass1"] + inj_arr["mass2"])**0.2)
inj_eta = inj_arr["mass1"] * inj_arr["mass2"] / (inj_arr["mass1"] + inj_arr["mass2"])**2
tmplt_M = tmplt_arr["mass1"] + tmplt_arr["mass2"]
tmplt_eta = tmplt_arr["mass1"] * tmplt_arr["mass2"] / (tmplt_arr["mass1"] + tmplt_arr["mass2"])**2
inj_mass_ratio = inj_arr["mass1"] / inj_arr["mass2"]

#
# compute effective/reduced spin parameter for templates
#
if tmplt_approx == "TaylorF2RedSpin":
    tmplt_chi_label = "\chi_\mathrm{red}"
    tmplt_chi = [SimInspiralTaylorF2ReducedSpinComputeChi(float(row["mass1"]), float(row["mass2"]), float(row["spin1z"]), float(row["spin2z"])) for row in tmplt_arr]
else: # default to effective spin
    tmplt_chi_label = "\chi_\mathrm{eff}"
    tmplt_chi = [SimIMRPhenomBComputeChi(float(row["mass1"]), float(row["mass2"]), float(row["spin1z"]), float(row["spin2z"])) for row in tmplt_arr]

# FIXME hack
# inj_dur = [SimIMRSEOBNRv4ROMTimeOfFrequency(flow, float(row["mass1"]) * MSUN_SI, float(row["mass2"]) * MSUN_SI, float(row["spin1z"]), float(row["spin2z"])) for row in inj_arr]


#
# compute effective/reduced spin parameter for injections
#
if inj_approx == "TaylorF2RedSpin" or "SpinTaylorT5" in inj_approx: # reduced spin
    inj_chi_label = "\chi_\mathrm{red}"
    inj_chi = [SimInspiralTaylorF2ReducedSpinComputeChi(float(row["mass1"]), float(row["mass2"]), float(row["spin1z"]), float(row["spin2z"])) for row in inj_arr]
elif "SpinTaylorT4" in inj_approx: # reduced spin (requires coordinate transformation)
    inj_chi_label = "\chi_\mathrm{red}"
    chi1 = [row["spin1x"] *np.sin(row["inclination"]) + row["spin1z"] *np.cos(row["inclination"]) for row in inj_arr]
    chi2 = [row["spin2x"] *np.sin(row["inclination"]) + row["spin2z"] *np.cos(row["inclination"]) for row in inj_arr]
    inj_chi = [SimIMRPhenomBComputeChi(float(row["mass1"]), float(row["mass2"]), s1z, s2z) for row, s1z, s2z in zip(inj_arr, chi1, chi2)]
else: # default to effective spin
    inj_chi_label = "\chi_\mathrm{eff}"
    inj_chi = [SimIMRPhenomBComputeChi(float(row["mass1"]), float(row["mass2"]), float(row["spin1z"]), float(row["spin2z"])) for row in inj_arr]

    # IMRPhenomP uses yet another coordinate convention
    if inj_approx == "IMRPhenomP":
        inj_chi *= np.cos(inj_arr["inclination"])


smallest_match = match.min()

from matplotlib.figure import Figure
from matplotlib.backends.backend_agg import FigureCanvasAgg as FigureCanvas

# FIXME
NAME = 'SSM_OFFLINE_HIGH_HIGH'  


mismatch = 1 - match

# plots

mismatch.sort()
match.sort()
percent = np.arange(1, len(mismatch)+1) / len(mismatch)
mm90 = mismatch[np.searchsorted(percent, 0.90)]
fig = Figure()
ax = fig.add_axes((0.1, 0.1, 0.85, 0.85), xscale="log", yscale="log")
ax.plot(mismatch, np.arange(len(mismatch)) / len(mismatch))
ax.vlines(mm90, np.power(10,0), 1, linestyles = 'dashed')
ax.plot((mm90, mm90), (0, 1), "k--")
#ax.text(4.5e-1, 2e-4,r'$90\%$') #,rotation=90) #mm90+np.power(10,-1.0), np.power(10,-4.0)
# ax.set_xlim([1.0*np.power(10,-4.0), 1.2*np.power(10,0)])
# ax.set_ylim([1.0*np.power(10,-4.0), 1.2*np.power(10,0)])
ax.set_xlabel('mismatch (1 - fitting factor)', fontsize=12)
ax.set_ylabel('Fraction of injections', fontsize=12)
#ax.set_title(r'90th percentile match = %.4f' % (min_match), fontsize=10)
ax.text(2.1e-2, 2e-5, r'90th percentile match = %.4f' % (min_match), fontsize=8, rotation=90)
ax.tick_params(axis='x', labelsize=12)
ax.tick_params(axis='y', labelsize=12)
ax.grid(True)
canvas = FigureCanvas(fig)
fig.savefig(NAME+"_match_cummulative.png", bbox_inches='tight')


==> scripts/offline_ssm_bank/sbank_plot_sim_ssm_offline_joint_cumulative <==
# Copyright (C) 2011  Nickolas Fotopoulos
# Copyright (C) 2011-2017  Stephen Privitera
#
# This program is free software; you can redistribute it and/or modify it
# under the terms of the GNU General Public License as published by the
# Free Software Foundation; either version 2 of the License, or (at your
# option) any later version.
#
# This program is distributed in the hope that it will be useful, but
# WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the GNU General
# Public License for more details.
#
# You should have received a copy of the GNU General Public License along
# with this program; if not, write to the Free Software Foundation, Inc.,
# 51 Franklin Street, Fifth Floor, Boston, MA  02110-1301, USA.

from __future__ import division
from math import ceil, floor, log10
import sys
import os
import warnings
import numpy as np
import matplotlib
matplotlib.use("Agg")
import matplotlib.pyplot as plt
#plt.rcParams["font.family"] = "serif"
plt.rcParams.update({"font.family": 'serif', 'font.size':10})
plt.rcParams['figure.figsize'] = [4, 3] 
plt.rcParams['figure.dpi'] =  300
plt.rcParams['savefig.dpi'] = 300
from optparse import OptionParser

from h5py import File as H5File

def parse_command_line():
    parser = OptionParser(description = __doc__)
    parser.add_option("--name", metavar = "name", default = "cumulative_plot", help = "Provide name of output plot.")
    parser.add_option("--high-high", metavar = "filename", help = "Provide high-high banksim h5 files.")
    parser.add_option("--high-low", metavar = "filename", help = "Provide high-low banksim h5 files.")
    parser.add_option("--low-low", metavar = "filename", help = "Provide low-low banksim h5 files.")

    options, filenames = parser.parse_args()
    return options, filenames

options, filenames = parse_command_line()

# grab data
high_high = None
high_low = None
low_low = None

match = None

def open_h5_file(filename, match_param):
    with H5File(filename, 'r') as h5file:
        match_param = np.array(h5file['/match_map'])
    match = match_param["match"]
    order = match.argsort()[::-1]
    match = match[order]
    min_match = match[int(floor(len(match)*0.99))]
    mismatch = 1 - match
    return match, min_match, mismatch

def open_h5_files(filename_hh, filename_hl, filename_ll, match_param):
    for fname in [filename_hh, filename_hl, filename_ll]:
        with H5File(fname, 'r') as h5file:
            if match_param is None:
                match_param = np.array(h5file['/match_map'])
            else:
                match_param = np.concatenate((np.array(h5file["/match_map"]), match_param))
    match = match_param["match"]
    order = match.argsort()[::-1]
    match = match[order]
    min_match = match[int(floor(len(match)*0.9))]
    mismatch = 1 - match
    return match, min_match, mismatch

match, min_match, mismatch = open_h5_files(options.high_high, options.high_low, options.low_low, match)

flow = 45 # FIXME

from matplotlib.figure import Figure
from matplotlib.backends.backend_agg import FigureCanvasAgg as FigureCanvas

mismatch.sort()
match.sort()
percent = np.arange(1, len(mismatch)+1) / len(mismatch)
mm90 = mismatch[np.searchsorted(percent, 0.90)]
fig = Figure()
ax = fig.add_axes((0.1, 0.1, 0.85, 0.85), xscale="log", yscale="log")
ax.plot(mismatch, np.arange(len(mismatch)) / len(mismatch))
ax.vlines(mm90, np.power(10,0), 1, linestyles = 'dashed')
ax.plot((mm90, mm90), (0, 1), "k--")
ax.text(3.2e-2, 2e-4,r'$90\%$') #,rotation=90)
# ax.set_xlim([1.0*np.power(10,-4.0), 1.2*np.power(10,0)])
# ax.set_ylim([1.0*np.power(10,-4.0), 1.2*np.power(10,0)])
ax.set_xlabel('mismatch (1 - fitting factor)', fontsize=10)
ax.set_ylabel('Fraction of injections', fontsize=10)
ax.set_title(r'90th percentile match = %.4f' % (min_match), fontsize=10)
ax.tick_params(axis='x', labelsize=10) 
ax.tick_params(axis='y', labelsize=10)
ax.grid(True)
canvas = FigureCanvas(fig)
fig.savefig(options.name+"_joint_cumulative.png", bbox_inches='tight')



==> scripts/online_ssm_bank/sbank_plot_sim_ssm_online <==
# Copyright (C) 2011  Nickolas Fotopoulos
# Copyright (C) 2011-2017  Stephen Privitera
#
# This program is free software; you can redistribute it and/or modify it
# under the terms of the GNU General Public License as published by the
# Free Software Foundation; either version 2 of the License, or (at your
# option) any later version.
#
# This program is distributed in the hope that it will be useful, but
# WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the GNU General
# Public License for more details.
#
# You should have received a copy of the GNU General Public License along
# with this program; if not, write to the Free Software Foundation, Inc.,
# 51 Franklin Street, Fifth Floor, Boston, MA  02110-1301, USA.

from __future__ import division
from math import ceil, floor, log10
import sys
import os
import warnings
import numpy as np
import matplotlib
matplotlib.use("Agg")
import matplotlib.pyplot as plt
#plt.rcParams["font.family"] = "serif"
plt.rcParams.update({"font.family": 'serif', 'font.size':10})
plt.rcParams['figure.figsize'] = [3.375, 2.531]
from lalsimulation import SimInspiralTaylorF2ReducedSpinComputeChi, SimIMRPhenomBComputeChi, SimIMRSEOBNRv4ROMTimeOfFrequency

from h5py import File as H5File

warnings.warn(
    "this script has been moved into the independent `sbank` project, "
    "see https://pypi.org/project/sbank/ for details, and will be "
    "removed from lalapps in an upcoming release",
    DeprecationWarning,
)


def find_process_id(process_table, prog_name):
    for program, pid in process_table["program", "process_id"]:
        if program == prog_name:
            return pid
    return None

def find_process_param(pp_table, process_id, param):
    for pid, row_param, value in pp_table["process_id", "param", "value"]:
        if pid == process_id and row_param == param:
            return value

# grab data
match = None
for fname in sys.argv[1:]:
    with H5File(fname, "r") as h5file:

        if match is None:
            match = np.array(h5file["/match_map"])
            inj_arr = np.array(h5file["/sim_inspiral"])
            tmplt_arr = np.array(h5file["/sngl_inspiral"])

        else:
            match = np.concatenate((np.array(h5file["/match_map"]), match))
            tmplt_arr = np.concatenate((np.array(h5file["/sngl_inspiral"]), tmplt_arr))
            inj_arr = np.concatenate((np.array(h5file["/sim_inspiral"]), inj_arr))

inj_sigmasq = match["inj_sigmasq"]
match = match["match"]

order = match.argsort()[::-1]
match = match[order]
inj_arr = inj_arr[order]
tmplt_arr = tmplt_arr[order]

inj_approx = "FIXME"
tmplt_approx = "FIXME"
flow = 30 # FIXME

# derived quantities
# NB: Named fields in dtypes (see ligolw_table_to_array in lalapps_cbc_sbank_sim)
# allow dict-like access to columns: e.g. arr["mass1"].
min_match = match[int(floor(len(match)*0.9))]
inj_M = inj_arr["mass1"] + inj_arr["mass2"] #total mass
inj_Mc = ((inj_arr["mass1"] * inj_arr["mass2"])**0.6) / ((inj_arr["mass1"] + inj_arr["mass2"])**0.2)
inj_eta = inj_arr["mass1"] * inj_arr["mass2"] / (inj_arr["mass1"] + inj_arr["mass2"])**2
tmplt_M = tmplt_arr["mass1"] + tmplt_arr["mass2"]
tmplt_eta = tmplt_arr["mass1"] * tmplt_arr["mass2"] / (tmplt_arr["mass1"] + tmplt_arr["mass2"])**2
inj_mass_ratio = inj_arr["mass1"] / inj_arr["mass2"]

#
# compute effective/reduced spin parameter for templates
#
if tmplt_approx == "TaylorF2RedSpin":
    tmplt_chi_label = "\chi_\mathrm{red}"
    tmplt_chi = [SimInspiralTaylorF2ReducedSpinComputeChi(float(row["mass1"]), float(row["mass2"]), float(row["spin1z"]), float(row["spin2z"])) for row in tmplt_arr]
else: # default to effective spin
    tmplt_chi_label = "\chi_\mathrm{eff}"
    tmplt_chi = [SimIMRPhenomBComputeChi(float(row["mass1"]), float(row["mass2"]), float(row["spin1z"]), float(row["spin2z"])) for row in tmplt_arr]

# FIXME hack
# inj_dur = [SimIMRSEOBNRv4ROMTimeOfFrequency(flow, float(row["mass1"]) * MSUN_SI, float(row["mass2"]) * MSUN_SI, float(row["spin1z"]), float(row["spin2z"])) for row in inj_arr]


#
# compute effective/reduced spin parameter for injections
#
if inj_approx == "TaylorF2RedSpin" or "SpinTaylorT5" in inj_approx: # reduced spin
    inj_chi_label = "\chi_\mathrm{red}"
    inj_chi = [SimInspiralTaylorF2ReducedSpinComputeChi(float(row["mass1"]), float(row["mass2"]), float(row["spin1z"]), float(row["spin2z"])) for row in inj_arr]
elif "SpinTaylorT4" in inj_approx: # reduced spin (requires coordinate transformation)
    inj_chi_label = "\chi_\mathrm{red}"
    chi1 = [row["spin1x"] *np.sin(row["inclination"]) + row["spin1z"] *np.cos(row["inclination"]) for row in inj_arr]
    chi2 = [row["spin2x"] *np.sin(row["inclination"]) + row["spin2z"] *np.cos(row["inclination"]) for row in inj_arr]
    inj_chi = [SimIMRPhenomBComputeChi(float(row["mass1"]), float(row["mass2"]), s1z, s2z) for row, s1z, s2z in zip(inj_arr, chi1, chi2)]
else: # default to effective spin
    inj_chi_label = "\chi_\mathrm{eff}"
    inj_chi = [SimIMRPhenomBComputeChi(float(row["mass1"]), float(row["mass2"]), float(row["spin1z"]), float(row["spin2z"])) for row in inj_arr]

    # IMRPhenomP uses yet another coordinate convention
    if inj_approx == "IMRPhenomP":
        inj_chi *= np.cos(inj_arr["inclination"])


smallest_match = match.min()

from matplotlib.figure import Figure
from matplotlib.backends.backend_agg import FigureCanvasAgg as FigureCanvas

# FIXME
NAME = 'SSM_ONLINE_BNS_LOW'
# MAX_MISMATCH =  #max(mismatch)+numpy.power(10,-3.0)
# BBH, NSBH_LOW, NSBH_HIGH: 1.0, BNS_LOW, BNS_HIGH: 0.6
MAX_MISMATCH = 0.6

import numpy
mismatch = 1 - match
mismatch_mapped = mismatch
mismatch_mapped[mismatch_mapped < 0.01] = 0.01


# plots

fig = Figure()
ax = fig.add_subplot(111)
collection = ax.scatter(inj_Mc, inj_chi, c=mismatch_mapped, s=4., linewidth=0, alpha=0.25, norm=matplotlib.colors.LogNorm(0.0+numpy.power(10,-2.0), MAX_MISMATCH))
ax.set_xlabel("Injected Chirp Mass", fontsize=12)
ax.set_ylabel("Injected $%s$" % inj_chi_label, fontsize=12)
ax.tick_params(axis='x', labelsize=12)
ax.tick_params(axis='y', labelsize=12)
ax.grid(True)
# BBH
# ax.set_xlim([0.40, 2.47])
# ax.set_ylim([-0.325, 0.325])
# NSBH_LOW, NSBH_HIGH
# ax.set_xlim([1.35, 4.75])
# ax.set_ylim([-1.05, 1.05])
# BNS_LOW:
ax.set_xlim([0.75, 2.75])
ax.set_ylim([-0.055, 0.055])
# BNS_HIGH:
# ax.set_xlim([0.75, 2.75])
# ax.set_ylim([-0.51, 0.51])
ax.margins(x=1.0,y=1.0)
fig.colorbar(collection, ax=ax).set_label("mismatch (1 - fitting factor)", fontsize=12)
canvas = FigureCanvas(fig)
fig.savefig(NAME+"_match_vs_injMc_vs_injchi.png", bbox_inches='tight', figsize=(3.375, 2.531))




==> scripts/online_ssm_bank/sbank_plot_sim_ssm_online_cumulative <==
# Copyright (C) 2011  Nickolas Fotopoulos
# Copyright (C) 2011-2017  Stephen Privitera
#
# This program is free software; you can redistribute it and/or modify it
# under the terms of the GNU General Public License as published by the
# Free Software Foundation; either version 2 of the License, or (at your
# option) any later version.
#
# This program is distributed in the hope that it will be useful, but
# WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the GNU General
# Public License for more details.
#
# You should have received a copy of the GNU General Public License along
# with this program; if not, write to the Free Software Foundation, Inc.,
# 51 Franklin Street, Fifth Floor, Boston, MA  02110-1301, USA.

from __future__ import division
from math import ceil, floor, log10
import sys
import os
import warnings
import numpy as np
import matplotlib
matplotlib.use("Agg")
import matplotlib.pyplot as plt
#plt.rcParams["font.family"] = "serif"
plt.rcParams.update({"font.family": 'serif', 'font.size':10})
plt.rcParams['figure.figsize'] = [3.375, 2.531]
from lalsimulation import SimInspiralTaylorF2ReducedSpinComputeChi, SimIMRPhenomBComputeChi, SimIMRSEOBNRv4ROMTimeOfFrequency

from h5py import File as H5File

warnings.warn(
    "this script has been moved into the independent `sbank` project, "
    "see https://pypi.org/project/sbank/ for details, and will be "
    "removed from lalapps in an upcoming release",
    DeprecationWarning,
)


def find_process_id(process_table, prog_name):
    for program, pid in process_table["program", "process_id"]:
        if program == prog_name:
            return pid
    return None

def find_process_param(pp_table, process_id, param):
    for pid, row_param, value in pp_table["process_id", "param", "value"]:
        if pid == process_id and row_param == param:
            return value

# grab data
match = None
for fname in sys.argv[1:]:
    with H5File(fname, "r") as h5file:

        if match is None:
            match = np.array(h5file["/match_map"])
            inj_arr = np.array(h5file["/sim_inspiral"])
            tmplt_arr = np.array(h5file["/sngl_inspiral"])

        else:
            match = np.concatenate((np.array(h5file["/match_map"]), match))
            tmplt_arr = np.concatenate((np.array(h5file["/sngl_inspiral"]), tmplt_arr))
            inj_arr = np.concatenate((np.array(h5file["/sim_inspiral"]), inj_arr))

inj_sigmasq = match["inj_sigmasq"]
match = match["match"]

order = match.argsort()[::-1]
match = match[order]
inj_arr = inj_arr[order]
tmplt_arr = tmplt_arr[order]

inj_approx = "FIXME"
tmplt_approx = "FIXME"
flow = 30 # FIXME

# derived quantities
# NB: Named fields in dtypes (see ligolw_table_to_array in lalapps_cbc_sbank_sim)
# allow dict-like access to columns: e.g. arr["mass1"].
min_match = match[int(floor(len(match)*0.9))]
inj_M = inj_arr["mass1"] + inj_arr["mass2"] #total mass
inj_Mc = ((inj_arr["mass1"] * inj_arr["mass2"])**0.6) / ((inj_arr["mass1"] + inj_arr["mass2"])**0.2)
inj_eta = inj_arr["mass1"] * inj_arr["mass2"] / (inj_arr["mass1"] + inj_arr["mass2"])**2
tmplt_M = tmplt_arr["mass1"] + tmplt_arr["mass2"]
tmplt_eta = tmplt_arr["mass1"] * tmplt_arr["mass2"] / (tmplt_arr["mass1"] + tmplt_arr["mass2"])**2
inj_mass_ratio = inj_arr["mass1"] / inj_arr["mass2"]

#
# compute effective/reduced spin parameter for templates
#
if tmplt_approx == "TaylorF2RedSpin":
    tmplt_chi_label = "\chi_\mathrm{red}"
    tmplt_chi = [SimInspiralTaylorF2ReducedSpinComputeChi(float(row["mass1"]), float(row["mass2"]), float(row["spin1z"]), float(row["spin2z"])) for row in tmplt_arr]
else: # default to effective spin
    tmplt_chi_label = "\chi_\mathrm{eff}"
    tmplt_chi = [SimIMRPhenomBComputeChi(float(row["mass1"]), float(row["mass2"]), float(row["spin1z"]), float(row["spin2z"])) for row in tmplt_arr]

# FIXME hack
# inj_dur = [SimIMRSEOBNRv4ROMTimeOfFrequency(flow, float(row["mass1"]) * MSUN_SI, float(row["mass2"]) * MSUN_SI, float(row["spin1z"]), float(row["spin2z"])) for row in inj_arr]


#
# compute effective/reduced spin parameter for injections
#
if inj_approx == "TaylorF2RedSpin" or "SpinTaylorT5" in inj_approx: # reduced spin
    inj_chi_label = "\chi_\mathrm{red}"
    inj_chi = [SimInspiralTaylorF2ReducedSpinComputeChi(float(row["mass1"]), float(row["mass2"]), float(row["spin1z"]), float(row["spin2z"])) for row in inj_arr]
elif "SpinTaylorT4" in inj_approx: # reduced spin (requires coordinate transformation)
    inj_chi_label = "\chi_\mathrm{red}"
    chi1 = [row["spin1x"] *np.sin(row["inclination"]) + row["spin1z"] *np.cos(row["inclination"]) for row in inj_arr]
    chi2 = [row["spin2x"] *np.sin(row["inclination"]) + row["spin2z"] *np.cos(row["inclination"]) for row in inj_arr]
    inj_chi = [SimIMRPhenomBComputeChi(float(row["mass1"]), float(row["mass2"]), s1z, s2z) for row, s1z, s2z in zip(inj_arr, chi1, chi2)]
else: # default to effective spin
    inj_chi_label = "\chi_\mathrm{eff}"
    inj_chi = [SimIMRPhenomBComputeChi(float(row["mass1"]), float(row["mass2"]), float(row["spin1z"]), float(row["spin2z"])) for row in inj_arr]

    # IMRPhenomP uses yet another coordinate convention
    if inj_approx == "IMRPhenomP":
        inj_chi *= np.cos(inj_arr["inclination"])


smallest_match = match.min()

from matplotlib.figure import Figure
from matplotlib.backends.backend_agg import FigureCanvasAgg as FigureCanvas

# FIXME
NAME = 'SSM_ONLINE_BBH'

import numpy
mismatch = 1 - match

# plots

mismatch.sort()
percent = np.arange(1, len(mismatch)+1) / len(mismatch)
mm90 = mismatch[np.searchsorted(percent, 0.90)]
fig = Figure()
ax = fig.add_axes((0.1, 0.1, 0.85, 0.85), xscale="log", yscale="log")
#ax = fig.add_subplot(111)
#ax.set_xscale("log")
#ax.set_yscale("log")
ax.plot(mismatch, 1.0 - (np.arange(len(mismatch)) / len(mismatch)))
#ax.vlines(mm90, np.power(10,0), 1, linestyles = 'dashed')
#ax.plot((mm90, mm90), (0, 1), "k--")
#ax.text(mm90+np.power(10,-3.0), np.power(10,-4.0),'90%', fontsize = 12) #,rotation=90)
#ax.set_xlim([9.5*np.power(10,-3.0), np.power(10,-1.0)])
ax.set_xlabel('mismatch (1 - fitting factor)', fontsize=12)
ax.set_ylabel('fraction above given mismatch', fontsize=12)
ax.set_title(r'$N_\mathrm{inj}=%d$, 90th percentile=%.4f' % (len(match), min_match,), fontsize=12)
ax.tick_params(axis='x', labelsize=12)
ax.tick_params(axis='y', labelsize=12)
ax.grid(True)
canvas = FigureCanvas(fig)
fig.savefig(NAME+"_match_cummulative.png", bbox_inches='tight', figsize=(3.375, 2.531))

